Modeling Topical Coherence in Discourse without Supervision

Coherence of text is an important attribute to be measured for both manually and automatically generated discourse; but well-defined quantitative metrics for it are still elusive. In this paper, we present a metric for scoring topical coherence of an input paragraph on a real-valued scale by analyzing its underlying topical structure. We first extract all possible topics that the sentences of a paragraph of text are related to. Coherence of this text is then measured by computing: (a) the degree of uncertainty of the topics with respect to the paragraph, and (b) the relatedness between these topics. All components of our modular framework rely only on unlabeled data and WordNet, thus making it completely unsupervised, which is an important feature for general-purpose usage of any metric. Experiments are conducted on two datasets - a publicly available dataset for essay grading (representing human discourse), and a synthetic dataset constructed by mixing content from multiple paragraphs covering diverse topics. Our evaluation shows that the measured coherence scores are positively correlated with the ground truth for both the datasets. Further validation to our coherence scores is provided by conducting human evaluation on the synthetic data, showing a significant agreement of 79.3%

==> 3_central.tex <==
\section{Formulation}
\label{sec:central}
Based on the earlier discussion, a \textit{prima-facie} formulation of coherence of a paragraph (denoted as $C$) can be proposed assuming that $C$ varies linearly and positively with: (a) to what degree of certainty topics in the paragraph (denoted as $T$) are supported by its constituent sentences (denoted by $E(T)$), and (b) to what extent these topics are related to each other (denoted by $\lambda(T)$. Mathematically,
\begin{equation}
C = \kappa E(T) \times \lambda (T)
\label{eq:main_coh}
\end{equation}
For empirical purposes, $\kappa$, the constant term can be set to $1$.

We now proceed to the next section where we describe each components of our formula.

==> 5_algorithm.tex <==
\section{Scoring Algorithm}
\label{sec:algorithm}
\algsetup{indent=2em}
\newcommand{\sentiaggr}{\ensuremath{\mbox{\sc The Overall Approach}}}
\begin{algorithm*}[t]
\caption{$\sentiaggr$}
\label{alg:sentiaggr}

%\begin{multicols}{2}
\begin{algorithmic}[1]
%\footnotesize
\STATE $\mathcal{G}(\mathcal{V},\mathcal{E})$ $\gets$ OntologyGraphCreate()
\newline

\FOR {each vertex $v \in \mathcal{G}$}
	\STATE centrality($v$) $\gets$ centrality measure value of vertex $v$ in graph $\mathcal{G}$
\ENDFOR
\newline

\STATE $total\_senti \gets 0$
\FOR {each user review $\mathcal{R}$}
	\STATE extract entities $\mathcal{T}$ from $\mathcal{R}$
	\STATE perform dependency parsing of $\mathcal{R}$
	\STATE $user\_senti \gets 0$
	\FOR {each dependency $\mathcal{D}$ where $f = headword(\mathcal{D}) \in$ the full feature/aspect set $\mathcal{F}$}
		\STATE ({\bf REM} Each headword represents an aspect of the review)
		\STATE $dep\_senti(f) \gets 0$
		\FOR {each word-concept $w \in \mathcal{D}$}
			\STATE $dep\_senti(f) \gets dep\_senti(f) + Sentiment(w)$
		\ENDFOR
		\IF {$f \in \mathcal{V}$}
			\STATE $user\_senti \gets user\_senti + dep\_senti(f) \times centrality(f)$
		%\ELSE
		%	\STATE $m \gets embedding(f,\mathcal{R})$
		%	\STATE \textbf{ABHIJIT, how do we replace the centrality of f by the value of embedding? Please add it HERE}
		\ENDIF
	\ENDFOR
	\STATE $user\_senti\_set \gets user\_senti\_set~ \cup <\mathcal{R},user\_senti>$
	\STATE $total\_senti \gets total\_senti + user\_senti$
\ENDFOR
\renewcommand{\algorithmicreturn}{\textbf{Output:}}
\RETURN $total\_senti$, $user\_senti\_set$
\newline

\STATE {\it function} {\bf Sentiment(Word Concept $w$)}:
\STATE return Sentiment\_Dictionary\_Lookup($w$) ({\bf REM} SentiWordNet, Bing Liu {\it etc.})
\newline
\end{algorithmic}
%\end{multicols}
\end{algorithm*}


